Semi-supervised clustering methods

Cluster analysis methods seek to partition a data set into homogeneous subgroups. It is useful in a wide variety of applications, including document processing and modern genetics. Conventional clustering methods are unsupervised, meaning that there is no outcome variable nor is anything known about the relationship between the observations in the data set. In many situations, however, information about the clusters is available in addition to the values of the features. For example, the cluster labels of some observations may be known, or certain observations may be known to belong to the same cluster. In other cases, one may wish to identify clusters that are associated with a particular outcome variable. This review describes several clustering algorithms (known as "semi-supervised clustering" methods) that can be applied in these situations. The majority of these methods are modifications of the popular k-means clustering method, and several of them will be described in detail. A brief description of some other semi-supervised clustering algorithms is also provided.

==> crossreflist.tex <==
\Crossrefs{CSA0001}{Pharmacokinetics}
\Crossrefs{CSF0001}{Computed tomography}
\Crossrefs{CSA0002}{Neurophysiology}
\Crossrefs{CSA0003}{Growth curves}
\Crossrefs{CSV0001}{Epidemiology}
\Crossrefs{CSA0004}{Computational biology}
\Crossrefs{CSF0002}{Axon}
\Crossrefs{CSA0005}{Chemometrics}
\Crossrefs{CSV0002}{Weather models and prediction}
\Crossrefs{CSA0006}{Climate models and prediction}
\Crossrefs{CSA0007}{Statistics in finance}
\Crossrefs{CSV0003}{Financial mathematics}
\Crossrefs{CSA0008}{Computational finance}
\Crossrefs{CSA0009}{Computational geometry}
\Crossrefs{CSA0010}{Graph layout}
\Crossrefs{CSA0011}{Statistics of shape}
\Crossrefs{CSA0012}{Interated function systems}
\Crossrefs{CSA0013}{Fractals}
\Crossrefs{CSA0014}{Delaunay triangulation}
\Crossrefs{CSF0003}{Convex hull}
\Crossrefs{CSV0004}{Computational mathematics}
\Crossrefs{CSA0015}{Statistical methods in seismology}
\Crossrefs{CSA0016}{Remote sensing}
\Crossrefs{CSF0004}{Geostatistics}
\Crossrefs{CSV0005}{Cartography}
\Crossrefs{CSA0017}{Public policy}
\Crossrefs{CSF0005}{Statistical and Applied Mathematical Sciences Institute}
\Crossrefs{CSF0006}{National Institutes of Health}
\Crossrefs{CSF0007}{National Institute of Statistical Sciences}
\Crossrefs{CSF0008}{National Institute of Standards and Technology}
\Crossrefs{CSF0009}{National Center for Atmospheric Research}
\Crossrefs{CSF0010}{National Cancer Institute}
\Crossrefs{CSF0011}{Los Alamos National Laboratory}
\Crossrefs{CSF0012}{Lawrence Livermore National Laboratory}
\Crossrefs{CSF0013}{Journal of Statistical Software}
\Crossrefs{CSF0014}{Journal of Computational and Graphical Statistics}
\Crossrefs{CSF0015}{Interface Symposium}
\Crossrefs{CSF0016}{Interface Foundation of North America}
\Crossrefs{CSF0017}{Computing Science and Statistics}
\Crossrefs{CSF0018}{Computational Statistics and Data Analysis (CSDA)}
\Crossrefs{CSF0019}{Computational Statistics (Journal)}
\Crossrefs{CSA0018}{COMPSTAT}
\Crossrefs{CSA0019}{Comprehensive R archive network}
\Crossrefs{CSF0020}{Committee on Applied and Theoretical Statistics}
\Crossrefs{CSF0021}{Center for Disease Control}
\Crossrefs{CSV0006}{Forensic science}
\Crossrefs{CSV0007}{Representation of color}
\Crossrefs{CSA0020}{Human perception and cognition}
\Crossrefs{CSF0022}{Graphical perception}
\Crossrefs{CSA0021}{Statistical analysis of evidence}
\Crossrefs{CSA0022}{Color perception}
\Crossrefs{CSF0023}{Bounded rationality}
\Crossrefs{CSF0024}{Positron emission tomography}
\Crossrefs{CSA0023}{Functional magnetic resonance imaging}
\Crossrefs{CSA0024}{Steganography}
\Crossrefs{CSA0025}{Multimedia}
\Crossrefs{CSA0026}{MPEG}
\Crossrefs{CSV0008}{Encryption}
\Crossrefs{CSV0009}{Cryptology}
\Crossrefs{CSV0010}{Coding theory}
\Crossrefs{CSA0027}{Ciphers}
\Crossrefs{CSF0025}{Bearings-only tracking}
\Crossrefs{CSV0011}{Statistical communication theory}
\Crossrefs{CSA0028}{Spread spectrum}
\Crossrefs{CSV0012}{Signal processing}
\Crossrefs{CSF0026}{Signal detection theory}
\Crossrefs{CSA0029}{Kalman filter}
\Crossrefs{CSA0030}{Filtering for time series and signals}
\Crossrefs{CSA0031}{Probabilistic expert systems}
\Crossrefs{CSV0013}{Expert systems}
\Crossrefs{CSV0014}{Artificial intelligence}
\Crossrefs{CSA0032}{Computer vision}
\Crossrefs{CSA0033}{Meta-analysis}
\Crossrefs{CSF0027}{Clinical trial}
\Crossrefs{CSV0015}{Dna microarray data}
\Crossrefs{CSV0016}{Bioinformatics}
\Crossrefs{CSA0034}{Gene expression profiles}
\Crossrefs{CSV0017}{Statistical genetics}
\Crossrefs{CSA0035}{Medical informatics}
\Crossrefs{CSA0036}{Healthcare data}
\Crossrefs{CSV0018}{Bayesian model choice}
\Crossrefs{CSA0037}{Bayesian model averaging}
\Crossrefs{CSV0019}{Bayesian networks}
\Crossrefs{CSA0038}{Bayesian nonparametric methods}
\Crossrefs{CSV0020}{Empirical Bayes}
\Crossrefs{CSF0028}{Belief function}
\Crossrefs{CSV0021}{Bayesian inference}
\Crossrefs{CSA0039}{Bayesian estimation}
\Crossrefs{CSF0029}{Bayesian data analysis}
\Crossrefs{CSF0030}{Bayesian computation}
\Crossrefs{CSA0040}{Bayesian classification}
\Crossrefs{CSV0022}{Bayes theorem}
\Crossrefs{CSV0023}{Gibbs sampling}
\Crossrefs{CSV0024}{Markov chain Monte Carlo}
\Crossrefs{CSV0025}{Distribution-free methods}
\Crossrefs{CSF0031}{Resampling}
\Crossrefs{CSV0026}{Jackknife}
\Crossrefs{CSV0027}{Bootstrap}
\Crossrefs{CSV0028}{Averaged shifted histogram}
\Crossrefs{CSA0041}{Finite mixture distributions}
\Crossrefs{CSA0042}{Nonparametric regression}
\Crossrefs{CSV0029}{Nonparametric curve estimation}
\Crossrefs{CSV0030}{Wavelet methods}
\Crossrefs{CSF0032}{Thin plate splines}
\Crossrefs{CSV0031}{Splines}
\Crossrefs{CSF0033}{Spline smoothing}
\Crossrefs{CSV0032}{Smoothing}
\Crossrefs{CSF0034}{Pearson family of distributions}
\Crossrefs{CSF0035}{L2E method}
\Crossrefs{CSA0043}{Kernel regression}
\Crossrefs{CSV0033}{Kernel density estimation}
\Crossrefs{CSA0044}{Johnson family of distributions}
\Crossrefs{CSF0036}{Histogram}
\Crossrefs{CSA0045}{Filtered kernel density estimation}
\Crossrefs{CSF0037}{Curve estimation}
\Crossrefs{CSF0038}{Burr family of distributions}
\Crossrefs{CSV0034}{Bandwidth in smoothing}
\Crossrefs{CSA0046}{Adaptive mixtures}
\Crossrefs{CSA0047}{Manifold learning}
\Crossrefs{CSV0035}{Computers and statistics}
\Crossrefs{CSA0048}{Computer-intensive methods}
\Crossrefs{CSA0049}{Multivariate space-time data}
\Crossrefs{CSA0050}{Multivariate density estimation}
\Crossrefs{CSV0036}{Multivariate analysis}
\Crossrefs{CSA0051}{Multiresolution analysis}
\Crossrefs{CSF0039}{Kolmogorov-Smirnov test}
\Crossrefs{CSA0052}{Computational rank-based statistics}
\Crossrefs{CSA0053}{Binning}
\Crossrefs{CSV0037}{Generalized cross validation}
\Crossrefs{CSV0038}{Cross validation}
\Crossrefs{CSA0054}{Operations research computations}
\Crossrefs{CSF0040}{Computer intensive tests}
\Crossrefs{CSA0055}{Outliers}
\Crossrefs{CSF0041}{Robust test}
\Crossrefs{CSV0039}{Robust methods}
\Crossrefs{CSA0056}{Minimum volume ellipsoid}
\Crossrefs{CSA0057}{Minimum covariance determinant}
\Crossrefs{CSA0058}{Influence}
\Crossrefs{CSV0040}{Detection of outliers}
\Crossrefs{CSF0042}{Breakdown value}
\Crossrefs{CSA0059}{Parallel computing}
\Crossrefs{CSA0060}{Computer performance measurement}
\Crossrefs{CSA0061}{Statistical computing}
\Crossrefs{CSA0062}{Algorithms for computational statistics}
\Crossrefs{CSF0043}{C programming language}
\Crossrefs{CSV0041}{Human computer interaction}
\Crossrefs{CSA0063}{Computing environments}
\Crossrefs{CSA0064}{Teraflop computer}
\Crossrefs{CSA0065}{Service oriented architecture}
\Crossrefs{CSA0066}{Biosurveillance}
\Crossrefs{CSA0067}{Data security}
\Crossrefs{CSA0068}{Disease mapping}
\Crossrefs{CSF0044}{Computer intrusion detection}
\Crossrefs{CSA0069}{Networks}
\Crossrefs{CSA0070}{Network traffic analysis}
\Crossrefs{CSA0071}{Network tomography}
\Crossrefs{CSA0072}{Internet traffic modeling}
\Crossrefs{CSF0045}{Fraud detection}
\Crossrefs{CSA0073}{Data confidentiality}
\Crossrefs{CSF0046}{Computer viruses}
\Crossrefs{CSA0074}{Computer security}
\Crossrefs{CSF0047}{Denial of service attack}
\Crossrefs{CSF0048}{Backscatter}
\Crossrefs{CSA0075}{Software reliability}
\Crossrefs{CSA0076}{Object oriented programming}
\Crossrefs{CSA0077}{Graphical user interface}
\Crossrefs{CSV0042}{Geographic information system}
\Crossrefs{CSF0049}{Vista}
\Crossrefs{CSV0043}{Statistical software}
\Crossrefs{CSV0044}{Software engineering}
\Crossrefs{CSF0050}{SAS}
\Crossrefs{CSA0078}{S}
\Crossrefs{CSF0051}{R graphics}
\Crossrefs{CSF0052}{Matlab library LIBRA}
\Crossrefs{CSF0053}{GENSTAT}
\Crossrefs{CSF0054}{Computer-aided instruction}
\Crossrefs{CSA0079}{Model-based clustering}
\Crossrefs{CSA0080}{Support vector machines}
\Crossrefs{CSF0055}{K-nearest neighbor}
\Crossrefs{CSA0081}{K-means clustering}
\Crossrefs{CSV0045}{Cluster analysis}
\Crossrefs{CSV0046}{Classification}
\Crossrefs{CSA0082}{Imputation}
\Crossrefs{CSV0047}{Data quality}
\Crossrefs{CSF0056}{Recursive partitioning}
\Crossrefs{CSF0057}{Record linkage}
\Crossrefs{CSA0083}{Handling of missing data points}
\Crossrefs{CSF0058}{Editing statistical data}
\Crossrefs{CSA0084}{Data compression}
\Crossrefs{CSA0085}{Data cleaning}
\Crossrefs{CSA0086}{Functional data analysis}
\Crossrefs{CSV0048}{Statistical data mining}
\Crossrefs{CSV0049}{Data mining}
\Crossrefs{CSF0059}{Google}
\Crossrefs{CSA0087}{Knowledge discovery in databases}
\Crossrefs{CSF0060}{Chi-squared automated interaction detector}
\Crossrefs{CSV0050}{Pattern recognition}
\Crossrefs{CSA0088}{Handwriting recongition}
\Crossrefs{CSA0089}{Feature extraction}
\Crossrefs{CSA0090}{Association rules}
\Crossrefs{CSA0091}{Streaming data}
\Crossrefs{CSF0061}{Hypertext}
\Crossrefs{CSA0092}{Text data mining}
\Crossrefs{CSA0093}{Speech recognition}
\Crossrefs{CSF0062}{Part-of-speech tagging}
\Crossrefs{CSA0094}{Latent semantic indexing}
\Crossrefs{CSA0095}{Information retrieval algorithms}
\Crossrefs{CSA0096}{Cross corpus discovery}
\Crossrefs{CSV0051}{Computational linguistics}
\Crossrefs{CSF0063}{Bigram proximity matrix}
\Crossrefs{CSV0052}{Categorical data}
\Crossrefs{CSV0053}{Data}
\Crossrefs{CSF0064}{Binary trees}
\Crossrefs{CSA0097}{Class cover catch digraphs}
\Crossrefs{CSA0098}{Random graphs for pattern recognition}
\Crossrefs{CSV0054}{Graph theory}
\Crossrefs{CSF0065}{Scan statistics on graphs}
\Crossrefs{CSA0099}{Random graphs}
\Crossrefs{CSF0066}{Directed graph}
\Crossrefs{CSF0067}{Bipartite matching}
\Crossrefs{CSF0068}{Spatial statistics}
\Crossrefs{CSF0069}{Spatial point processes}
\Crossrefs{CSF0070}{Spatial data analysis}
\Crossrefs{CSF0071}{Image restoration}
\Crossrefs{CSV0055}{Image processing}
\Crossrefs{CSA0100}{Image grand tour}
\Crossrefs{CSA0101}{Massive datasets}
\Crossrefs{CSF0072}{Lasso}
\Crossrefs{CSV0056}{Large datasets}
\Crossrefs{CSV0057}{Quantitative social sciences}
\Crossrefs{CSV0058}{Social network analysis}
\Crossrefs{CSF0073}{Change point detection}
\Crossrefs{CSV0059}{Autoregressive process}
\Crossrefs{CSV0060}{Autocovariance}
\Crossrefs{CSV0061}{Time series analysis}
\Crossrefs{CSA0102}{Computational methods in spectroscopy}
\Crossrefs{CSA0103}{Spectral estimation}
\Crossrefs{CSA0104}{Nonstationarity}
\Crossrefs{CSA0105}{Long-range dependence}
\Crossrefs{CSA0106}{Longitudinal data}
\Crossrefs{CSA0107}{Fractal Brownian motion}
\Crossrefs{CSV0062}{Missing data}
\Crossrefs{CSA0108}{Directional data}
\Crossrefs{CSA0109}{Circular data}
\Crossrefs{CSV0063}{Censored data}
\Crossrefs{CSV0064}{Interactive graphics}
\Crossrefs{CSV0065}{Information visualization}
\Crossrefs{CSF0074}{High-interaction graphics}
\Crossrefs{CSF0075}{Volume rendering}
\Crossrefs{CSF0076}{Rendering in computer graphics}
\Crossrefs{CSF0077}{Pixel rewrite}
\Crossrefs{CSA0110}{Computer aided design}
\Crossrefs{CSA0111}{3-d stereoscopic plots}
\Crossrefs{CSA0112}{Regression diagnostics}
\Crossrefs{CSV0066}{Diagnostics in data fitting}
\Crossrefs{CSF0078}{Cognostics}
\Crossrefs{CSF0079}{Sliced inverse regression}
\Crossrefs{CSV0067}{Multidimensional scaling}
\Crossrefs{CSF0080}{Dimension reduction}
\Crossrefs{CSA0113}{Visualization}
\Crossrefs{CSV0068}{Data visualization}
\Crossrefs{CSA0114}{Conditional chloropleth maps}
\Crossrefs{CSF0081}{Trellis display}
\Crossrefs{CSF0082}{Skyline plots}
\Crossrefs{CSF0083}{Chernoff faces}
\Crossrefs{CSF0084}{Brushing}
\Crossrefs{CSF0085}{Linked micromap plots}
\Crossrefs{CSA0115}{Grammar of graphics}
\Crossrefs{CSV0069}{Exploratory data analysis}
\Crossrefs{CSF0086}{Mosaic plots}
\Crossrefs{CSF0087}{MODRIAN}
\Crossrefs{CSF0088}{Manet}
\Crossrefs{CSA0116}{Scatterplots}
\Crossrefs{CSF0089}{Linked views}
\Crossrefs{CSF0090}{Linked low-dimensional views}
\Crossrefs{CSV0070}{Statistical graphics}
\Crossrefs{CSF0091}{Dynamic graphics}
\Crossrefs{CSA0117}{Data display}
\Crossrefs{CSF0092}{Casement display}
\Crossrefs{CSF0093}{Biplot}
\Crossrefs{CSF0094}{Binned bivariate scatterplot}
\Crossrefs{CSF0095}{Virtual reality modeling language}
\Crossrefs{CSA0118}{Virtual reality}
\Crossrefs{CSA0119}{Stereoscopic visualization}
\Crossrefs{CSA0120}{CAVE environment}
\Crossrefs{CSF0096}{Continuous animation}
\Crossrefs{CSF0097}{Color histogram}
\Crossrefs{CSF0098}{Chloropleth maps}
\Crossrefs{CSF0099}{Space-filling displays}
\Crossrefs{CSF0100}{Ggobi}
\Crossrefs{CSF0101}{Explor4}
\Crossrefs{CSF0102}{Crystalvision}
\Crossrefs{CSF0103}{Sizer}
\Crossrefs{CSA0121}{Scale space methods}
\Crossrefs{CSF0104}{BRUSH-TOUR}
\Crossrefs{CSA0122}{Andrews curves}
\Crossrefs{CSA0123}{Projection pursuit}
\Crossrefs{CSA0124}{Parallel coordinate displays and density plots}
\Crossrefs{CSA0125}{K-dimensional tours}
\Crossrefs{CSA0126}{Grand tour of high dimensional data}
\Crossrefs{CSA0127}{Relational databases}
\Crossrefs{CSF0105}{Decision trees}
\Crossrefs{CSV0071}{Classification and regression trees}
\Crossrefs{CSF0106}{Boosting}
\Crossrefs{CSF0107}{Bagging}
\Crossrefs{CSA0128}{Machine learning}
\Crossrefs{CSA0129}{Multivariate adaptive regression splines}
\Crossrefs{CSA0130}{Neural networks}
\Crossrefs{CSF0108}{Backfitting}
\Crossrefs{CSV0072}{Statistical learning}
\Crossrefs{CSV0073}{Agent based simulations}
\Crossrefs{CSV0074}{Generalized additive models}
\Crossrefs{CSV0075}{Statistical models}
\Crossrefs{CSV0076}{Model validity and verification}
\Crossrefs{CSA0131}{Model selection}
\Crossrefs{CSV0077}{Additive models}
\Crossrefs{CSA0132}{Adaptive model selection}
\Crossrefs{CSV0078}{Monte Carlo methods}
\Crossrefs{CSF0109}{Box-Muller transformation}
\Crossrefs{CSA0133}{Random number generation}
\Crossrefs{CSA0134}{Pseudo-random number generators}
\Crossrefs{CSF0110}{Antithetic random numbers}
\Crossrefs{CSA0135}{Validation of simulation models}
\Crossrefs{CSA0136}{Simulation methods}
\Crossrefs{CSV0079}{Modeling and simulation}
\Crossrefs{CSF0111}{Hierarchical models}
\Crossrefs{CSV0080}{Discrete event simulation}
\Crossrefs{CSV0081}{Computer models and statistics}
\Crossrefs{CSA0137}{Computer experiments, statistical analysis of}
\Crossrefs{CSF0112}{Computational feasibility}
\Crossrefs{CSA0138}{Computational complexity}
\Crossrefs{CSA0139}{Sparse matrix computations}
\Crossrefs{CSA0140}{Numerical analysis}
\Crossrefs{CSA0141}{N-dimensional quadrature}
\Crossrefs{CSV0082}{Gradient methods}
\Crossrefs{CSA0142}{Gaussian elimination}
\Crossrefs{CSF0113}{Cholesky decomposition}
\Crossrefs{CSV0083}{Evolutionary computation}
\Crossrefs{CSA0143}{Integer programming}
\Crossrefs{CSA0144}{Linear programming}
\Crossrefs{CSA0145}{Constrained optimization}
\Crossrefs{CSV0084}{Maximum likelihood estimation}
\Crossrefs{CSA0146}{Optimal experimental design}
\Crossrefs{CSF0114}{Log-linear model}
\Crossrefs{CSF0115}{Linear model}
\Crossrefs{CSA0147}{Generalized linear models}
\Crossrefs{CSV0085}{Fractional factorial design}
\Crossrefs{CSA0148}{Fixed and random effects models}
\Crossrefs{CSV0086}{Experimental design}
\Crossrefs{CSA0149}{Balanced incomplete block design}
\Crossrefs{CSV0087}{Analysis of variance}
\Crossrefs{CSV0088}{Expectation maximization}
\Crossrefs{CSF0116}{Kullback Liebler information}
\Crossrefs{CSV0089}{Information theory}
\Crossrefs{CSA0150}{Analog to Information}
\Crossrefs{CSA0151}{Akaike information criterion}
\Crossrefs{CSA0152}{Fuzzy set theory}
\Crossrefs{CSV0090}{Geometry in statistics}
\Crossrefs{CSV0091}{Combinatorics}
\Crossrefs{CSV0092}{Chaos and randomness}
\Crossrefs{CSA0153}{Nonparametric maximum likelihood}
\Crossrefs{CSF0117}{Rank methods}
\Crossrefs{CSV0093}{Nonparametric inference}
\Crossrefs{CSA0154}{Survival analysis}
\Crossrefs{CSF0118}{Statistical process control}
\Crossrefs{CSV0094}{Reliability}
\Crossrefs{CSF0119}{Quality control}
\Crossrefs{CSA0155}{Competing risks}
\Crossrefs{CSF0120}{Accelerated failure time}
\Crossrefs{CSA0156}{Sampling}
\Crossrefs{CSA0157}{Sample survey}
\Crossrefs{CSA0158}{Importance sampling}
\Crossrefs{CSF0121}{Adaptive sampling}
\Crossrefs{CSV0095}{Modes of inference}
\Crossrefs{CSF0122}{Convergence and asymptotics}
\Crossrefs{CSF0123}{Control chart}
\Crossrefs{CSA0159}{Partial least squares}
\Crossrefs{CSV0096}{Design of experiments}
\Crossrefs{CSV0097}{Principal component analysis}
\Crossrefs{CSF0124}{Concave minimization}
\Crossrefs{CSA0160}{Random fields}
\Crossrefs{CSA0161}{Prediction and forecasting}
\Crossrefs{CSV0098}{Discriminant analysis}
\Crossrefs{CSV0099}{Multiple regression}
\Crossrefs{CSF0125}{Penalized splines}
\Crossrefs{CSA0162}{Penalized methods}
\Crossrefs{CSA0163}{Normal mixtures}
\Crossrefs{CSV0100}{Semiparametric methods}
\Crossrefs{CSF0126}{Randomization}
\Crossrefs{CSA0164}{Contingency tables}
\Crossrefs{CSA0165}{Data masking for disclosure limitation}
\Crossrefs{CSF0127}{Tube theory}
\Crossrefs{CSF0128}{Subset selection}
\Crossrefs{CSA0166}{Stochastic calculus}
\Crossrefs{CSA0167}{Stochastic approximation}
\Crossrefs{CSA0168}{Stepwise regression}
\Crossrefs{CSF0129}{Stahel-Donoho estimator}
\Crossrefs{CSV0101}{Sequential methods}
\Crossrefs{CSF0130}{Ridge regression}
\Crossrefs{CSA0169}{Response surface methodology}
\Crossrefs{CSV0102}{Regression}
\Crossrefs{CSA0170}{Quantiles}
\Crossrefs{CSA0171}{Mode}
\Crossrefs{CSA0172}{Logistic regression}
\Crossrefs{CSV0103}{Linear regression}
\Crossrefs{CSA0173}{Least squares}
\Crossrefs{CSA0174}{Latent class analysis}
\Crossrefs{CSA0175}{Isotonic regression}
\Crossrefs{CSV0104}{Goodness-of-fit tests}
\Crossrefs{CSA0176}{Generalized estimating equations}
\Crossrefs{CSV0105}{Estimation}
\Crossrefs{CSA0177}{Errors in variables}
\Crossrefs{CSV0106}{Distribution functions and probability}
\Crossrefs{CSV0107}{Decision theory}
\Crossrefs{CSF0131}{Chi-bar squared distribution}
\Crossrefs{CSF0132}{Cauchy-Schwarz inequality}
\Crossrefs{CSF0133}{Brownian bridge}
\Crossrefs{CSV0108}{Asymptotic normality}
\Crossrefs{CSV0109}{Adaptive methods}
\Crossrefs{CSF0134}{Actuarial method}
\Crossrefs{CSV0110}{Acceptance sampling}
\Crossrefs{CSP0001}{History of statistics}
\Crossrefs{CSP0002}{Future of statistics}
\Crossrefs{CSA0178}{Discrete wavelet transform}
\Crossrefs{CSA0179}{Transformation of data}
\Crossrefs{CSF0135}{Box-Cox transformation}
\Crossrefs{CSF0136}{Neuron}
\Crossrefs{CSF0137}{Magnetic resonance imaging}
\Crossrefs{CSF0138}{Tessellation}
\Crossrefs{CSF0139}{Combining information}
\Crossrefs{CSF0140}{Digitized palomar sky survey}
\Crossrefs{CSF0141}{Mathematical Sciences Research Institute}
\Crossrefs{CSF0142}{RAND}
\Crossrefs{CSF0143}{Collected algorithms of the ACM}
\Crossrefs{CSF0144}{Journal of Statistical Computation and Simulation}
\Crossrefs{CSF0145}{International Association of Statistical Computing}
\Crossrefs{CSF0146}{Journal of the Pattern Recognition Society}
\Crossrefs{CSF0147}{Commumications in Statistics - Simulation and Computation}
\Crossrefs{CSF0148}{National Educational Longitudinal Study}
\Crossrefs{CSF0149}{Cognitive science}
\Crossrefs{CSF0150}{Huffman coding}
\Crossrefs{CSF0151}{Beamlets}
\Crossrefs{CSA0180}{Adaptive beamforming}
\Crossrefs{CSF0152}{Fast Fourier transform}
\Crossrefs{CSF0153}{JPEG}
\Crossrefs{CSF0154}{Bioassay}
\Crossrefs{CSF0155}{Cox model}
\Crossrefs{CSF0156}{Biological sequence data}
\Crossrefs{CSF0157}{Phylogeny reconstruction}
\Crossrefs{CSF0158}{Human Genome Project}
\Crossrefs{CSF0159}{Bayesian CART}
\Crossrefs{CSF0160}{Bezier curve}
\Crossrefs{CSF0161}{B-spline}
\Crossrefs{CSF0162}{Multivariate calibration}
\Crossrefs{CSF0163}{Multivariate contingency tables}
\Crossrefs{CSF0164}{Bin smoother}
\Crossrefs{CSF0165}{FORTRAN}
\Crossrefs{CSF0166}{Client-server architecture}
\Crossrefs{CSF0167}{Distributed grid-type architecture}
\Crossrefs{CSF0168}{Network monitoring}
\Crossrefs{CSF0169}{Firewall}
\Crossrefs{CSF0170}{Anomaly detection}
\Crossrefs{CSF0171}{Maple}
\Crossrefs{CSF0172}{BMDP - statistical software}
\Crossrefs{CSF0173}{MATLAB sofware}
\Crossrefs{CSF0174}{STATLIB}
\Crossrefs{CSF0175}{Guided tours}
\Crossrefs{CSF0176}{Adaboost}
\Crossrefs{CSF0177}{Yahoo!}
\Crossrefs{CSF0178}{Discounting older data}
\Crossrefs{CSF0179}{Natural language processing}
\Crossrefs{CSF0180}{Fisher's exact test}
\Crossrefs{CSF0181}{Categorical time series}
\Crossrefs{CSF0182}{Hyperspectral imagery data}
\Crossrefs{CSF0183}{Harmonic analysis}
\Crossrefs{CSF0184}{Extreme values}
\Crossrefs{CSF0185}{Arch and garch models}
\Crossrefs{CSF0186}{Birth-and-death process}
\Crossrefs{CSF0187}{3-d layering}
\Crossrefs{CSF0188}{Curse of dimensionality}
\Crossrefs{CSF0189}{Fractal dimension and estimation}
\Crossrefs{CSF0190}{Contour plot}
\Crossrefs{CSF0191}{Bertin's semiology}
\Crossrefs{CSF0192}{Multisensory virtual reality}
\Crossrefs{CSF0193}{Head-mounted device}
\Crossrefs{CSF0194}{Grand tour in Andrews curves}
\Crossrefs{CSF0195}{Random forests}
\Crossrefs{CSF0196}{AQ learning}
\Crossrefs{CSF0197}{Hidden Markov model}
\Crossrefs{CSF0198}{Backpropagation}
\Crossrefs{CSF0199}{Gauss-Newton algorithm}
\Crossrefs{CSF0200}{Conjugate gradient method}
\Crossrefs{CSF0201}{Combinatorial optimization}
\Crossrefs{CSF0202}{Interior point methods}
\Crossrefs{CSF0203}{Bayesian wavelet shrinkage}
\Crossrefs{CSF0204}{Entropy}
\Crossrefs{CSF0205}{Centroid}
\Crossrefs{CSF0206}{Calculus of variations}
\Crossrefs{CSF0207}{Combinatorial analysis}
\Crossrefs{CSF0208}{Banach space}
\Crossrefs{CSF0209}{Dirichlet process}
\Crossrefs{CSF0210}{Kaplan-Meier estimator}
\Crossrefs{CSF0211}{Hot deck method}
\Crossrefs{CSF0212}{Best linear unbiased estimator}
\Crossrefs{CSF0213}{Archaeometrics}
\Crossrefs{CSF0214}{Partial least squares regression}
\Crossrefs{CSF0215}{Calibration}
\Crossrefs{CSF0216}{Procrustes rotation}
\Crossrefs{CSF0217}{Capture-recapture}
\Crossrefs{CSF0218}{Canberra distance}
\Crossrefs{CSA0181}{Music}

